Unified Compression-Based Acceleration of Edit-Distance Computation

The edit distance problem is a classical fundamental problem in computer science in general, and in combinatorial pattern matching in particular. The standard dynamic programming solution for this problem computes the edit-distance between a pair of strings of total length O(N) in O(N^2) time. To this date, this quadratic upper-bound has never been substantially improved for general strings. However, there are known techniques for breaking this bound in case the strings are known to compress well under a particular compression scheme. The basic idea is to first compress the strings, and then to compute the edit distance between the compressed strings. As it turns out, practically all known o(N^2) edit-distance algorithms work, in some sense, under the same paradigm described above. It is therefore natural to ask whether there is a single edit-distance algorithm that works for strings which are compressed under any compression scheme. A rephrasing of this question is to ask whether a single algorithm can exploit the compressibility properties of strings under any compression method, even if each string is compressed using a different compression. In this paper we set out to answer this question by using straight line programs. These provide a generic platform for representing many popular compression schemes including the LZ-family, Run-Length Encoding, Byte-Pair Encoding, and dictionary methods. For two strings of total length N having straight-line program representations of total size n, we present an algorithm running in O(nN log(N/n)) time for computing the edit-distance of these two strings under any rational scoring function, and an O(n^{2/3}N^{4/3}) time algorithm for arbitrary scoring functions. Our new result, while providing a signi cant speed up for highly compressible strings, does not surpass the quadratic time bound even in the worst case scenario.

==> section3.1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Subsection: Beyond Levenshtein distance
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We next present a wider family of scoring functions to which our
speedup applies. Let $c$ be a natural number. A scoring function is
said have \emph{finite index $c$} with respect to a given alphabet
$\Sigma$, if there exist two partitions of $\Sigma$, each into at
most $c$ classes, such that:
\begin{itemize}
\item All replacements within each class in the first
partition have uniform cost.
\item All replacements between classes $i$ and $j$ in the first
partition have uniform cost for every $1\leq i,j \leq c$.
\item All insertions/deletions within each class in the
second partition have uniform cost.
\end{itemize}

\begin{example}
\label{Example: Finite index scoring function}%
Suppose $\Sigma$ is the English alphabet, and consider the scoring
function for which replacing two vowels costs 1, replacing two
consonants costs 3, and replacing a vowel with a consonant costs 5.
If this scoring function also uniformly assigns a cost of 3 for all
insertions/deletions of vowels, and a cost of 5 for all
insertions/deletions of consonants, then this scoring function has
finite index 2.
\end{example}

The Levenshtein distance is the simplest scoring function and it has
finite index 1. To cope with scoring functions of larger
finite index, we extend the $x$-signature so that it captures all
relevant information. Suppose our given scoring function has
finite index $c$ for some $c \in \mathbb{N}$, and for simplicity,
let us assume that both partitions are into exactly $c$ classes. Let
$A'$ and $B'$ be two substrings corresponding to some given
$x$-block $X$, and let $S$ denote the new signature we construct to
be associated with $A'$ and $B'$. The string $S$ is constructed over
an alphabet of size $O(x+c)$, and is the concatenation of three
substrings $S_1$, $S_2$, and $S_3$, each of length $O(x)$.

The substring $S_1$ encodes all matches between $A'$ and $B'$, or in
other words, all zero cost operations between letters of $A'$ and
$B'$. This is done by using the original $x$-signature of $A'$ and
$B'$. Substring $S_2$ encodes all replacements between $A'$ and
$B'$, and is simply the concatenation of $A'$ and $B'$ after
replacing all letters in class $i$ by the new letter $\sigma_i$ (see
Example~\ref{Example: Finite index signature}.). Finally, $S_3$
encodes all insertions/deletions and is created like $S_2$ with the
classes now defined by the second partition.

%and resembles the $x$-signature obtained from $A'$ and $B'$ after
%replacing all letters in class $i$ by the new letter $\sigma_i$. The
%only difference between $S_2$ and this $x$-signature is that in
%$S_2$ we also write $\sigma_i$ before we write the locations of
%$\sigma_i$ (see Example~\ref{Example: Finite-index signature}.).
%Finally, $S_3$ encodes all insertions/deletions and is created like
%$S_2$ with the classes now defined by the second partitioning.



\begin{example}
\label{Example: Finite index signature}%
Consider $A'$ = ``baller'' and $B'$ = ``bubble'' with the scoring
function of Example~\ref{Example: Finite index scoring function}
where consonants are denoted by `C` and vowels by 'V'. Then the
signature $S$ associated with $A'$ and $B'$ is given by $S =
S_1S_2S_3$, with $S_1 =$ ``$[(1)(1,3,4)][(3,4)(5)][(5)(6)]$'', and
$S_2 = S_3 =$ ``$[(\text{CVCCVC})(\text{CVCCCV})]$''.
\end{example}

It is easy to see that $S$, along with the difference vectors and
the upper-leftmost value of $X$, uniquely identify $X$. Furthermore,
like in the Levenshtein distance case, this signature is of length
$O(x)$, is over an alphabet of size $O(x+c)$, and can be computed in
linear time with respect to its length. Our speedup thus applies to
any finite index scoring function.

%It is easy to see that $S$, along with the difference vectors and
%the upper-leftmost value of $X$, uniquely identify $X$. This is
%because any edit operation on a pair of positions in $A'$ and $B'$
%not encoded in $S$ has uniform cost, and the cost of any other
%operation can be determined from $S$. Furthermore, like in the
%Levenshtein distance case, this signature is of length $O(x)$ and is
%over an alphabet of size $O(x+c)$. Finally, using essentially the
%same method for computing $x$-signatures described above, we can
%compute $S$ in linear time with respect to its length. Our speedup
%thus applies to every finite-index scoring function.


==> section7.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Section: Concluding Remarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
1. repository many times usage
2. parallel
3. compare two strings that each compress better with a different compression
4. $|A|^{0.57...}$


There are a few
open questions arising from our work:
\begin{itemize}
\item Can our first algorithm obtain an additional $\lg n$ speedup factor
like Masek and Paterson's algorithm by using similar ``indexing
by integers'' techniques?
%so that it is able to cope with arbitrary alphabets at no
%increase to its time complexity?
Or more generally, is there an $o(n^2\lg\lg n / \lg n)$
algorithm for edit-distance of strings over arbitrary alphabets?
\item Are there other types of scoring functions for which one can
compute the edit distance of two strings over an arbitrary alphabet
in sub-quadratic time?
\item Is there any way to extend our approach in
Section~\ref{Section: Extension for arbitrary scoring schemes} so
that it can handle alphabets of size $\omega(\lg n / \lg \lg n)$?
\end{itemize}
Finally, perhaps the most important open question in this context,
is whether there exists an $O(n^{2-\varepsilon})$ time edit distance
algorithm for any $\varepsilon > 0$, even for the case of binary
strings under the Levenshtein metric.

